NOMU: Neural Optimization-based Model Uncertainty

We study methods for estimating model uncertainty for neural networks (NNs) in regression. To isolate the effect of model uncertainty, we focus on a noiseless setting with scarce training data. We introduce five important desiderata regarding model uncertainty that any method should satisfy. However, we find that established benchmarks often fail to reliably capture some of these desiderata, even those that are required by Bayesian theory. To address this, we introduce a new approach for capturing model uncertainty for NNs, which we call Neural Optimization-based Model Uncertainty (NOMU). The main idea of NOMU is to design a network architecture consisting of two connected sub-NNs, one for model prediction and one for model uncertainty, and to train it using a carefully-designed loss function. Importantly, our design enforces that NOMU satisfies our five desiderata. Due to its modular architecture, NOMU can provide model uncertainty for any given (previously trained) NN if given access to its training data. We evaluate NOMU in various regressions tasks and noiseless Bayesian optimization (BO) with costly evaluations. In regression, NOMU performs at least as well as state-of-the-art methods. In BO, NOMU even outperforms all considered benchmarks.

==> tables/detailedBOFinalRegrets.tex <==
\begin{tabular}{lllllllllllll}
    \toprule
               &                        \multicolumn{1}{c}{\textbf{NOMU}} &                         \multicolumn{1}{c}{\textbf{NOMU}} &                          \multicolumn{1}{c}{\textbf{GP}} &                           \multicolumn{1}{c}{\textbf{GP}} &                          \multicolumn{1}{c}{\textbf{MCDO}} &                           \multicolumn{1}{c}{\textbf{MCDO}} &                          \multicolumn{1}{c}{\textbf{DE}} &                           \multicolumn{1}{c}{\textbf{DE}} &                         \multicolumn{1}{c}{\textbf{HDE}} &                          \multicolumn{1}{c}{\textbf{HDE}} &                         \multicolumn{1}{c}{\textbf{pGP}} &          \multicolumn{1}{c}{\textbf{RAND}} \\
              \textbf{Function} &                        \multicolumn{1}{c}{MW 0.05} &                         \multicolumn{1}{c}{MW 0.5} &                          \multicolumn{1}{c}{MW 0.05} &                           \multicolumn{1}{c}{MW 0.5} &                          \multicolumn{1}{c}{MW 0.05} &                           \multicolumn{1}{c}{MW 0.5} &                          \multicolumn{1}{c}{MW 0.05} &                           \multicolumn{1}{c}{MW 0.5} &                         \multicolumn{1}{c}{MW 0.05} &                          \multicolumn{1}{c}{MW 0.5} &                         \multicolumn{1}{c}{MW} &          \multicolumn{1}{c}{MW} \\
    \midrule
                Levy5D &                    $\num{2.12e-03}\pm\scriptsize\num{5.95e-04}$ & $\winc\num{1.52e-03}\pm\scriptsize\num{4.34e-04}$ & $\winc\num{1.10e-03}\pm\scriptsize\num{1.68e-04}$ &                    $\num{8.84e-03}\pm\scriptsize\num{1.15e-03}$ &                    $\num{1.98e-02}\pm\scriptsize\num{3.59e-03}$ &                    $\num{1.27e-02}\pm\scriptsize\num{2.57e-03}$ &                    $\num{7.09e-03}\pm\scriptsize\num{3.76e-03}$ &                    $\num{9.09e-02}\pm\scriptsize\num{9.16e-03}$ &                    $\num{4.48e-03}\pm\scriptsize\num{1.25e-03}$ &                    $\num{3.76e-03}\pm\scriptsize\num{1.22e-03}$ &                    $\num{6.25e-03}\pm\scriptsize\num{5.26e-04}$ & $\num{5.44e-02}\pm\scriptsize\num{4.22e-03}$ \\ 
          Rosenbrock5D & $\winc\num{1.75e-04}\pm\scriptsize\num{2.76e-05}$ & $\num{3.57e-04}\pm\scriptsize\num{6.39e-05}$ & $\num{3.62e-04}\pm\scriptsize\num{6.52e-05}$ & $\num{8.44e-04}\pm\scriptsize\num{1.62e-04}$ & $\num{2.83e-04}\pm\scriptsize\num{4.64e-05}$ & $\num{7.35e-04}\pm\scriptsize\num{1.08e-04}$ & $\winc\num{7.93e-04}\pm\scriptsize\num{7.74e-04}$ &                    $\num{5.96e-03}\pm\scriptsize\num{1.78e-03}$ & $\num{1.11e-03}\pm\scriptsize\num{7.25e-04}$ & $\num{5.02e-04}\pm\scriptsize\num{1.04e-04}$ & $\num{7.56e-04}\pm\scriptsize\num{8.13e-05}$ & $\num{4.73e-03}\pm\scriptsize\num{7.04e-04}$ \\ 
          G-Function5D &                    $\num{1.12e-01}\pm\scriptsize\num{1.99e-02}$ &                    $\num{1.06e-01}\pm\scriptsize\num{1.97e-02}$ &                    $\num{1.68e-01}\pm\scriptsize\num{1.62e-02}$ &                    $\num{2.60e-01}\pm\scriptsize\num{1.72e-02}$ & $\winc\num{2.66e-02}\pm\scriptsize\num{8.57e-03}$ &                    $\num{7.80e-02}\pm\scriptsize\num{8.82e-03}$ &                    $\num{1.88e-01}\pm\scriptsize\num{2.08e-02}$ &                    $\num{2.03e-01}\pm\scriptsize\num{2.20e-02}$ &                    $\num{1.35e-01}\pm\scriptsize\num{2.46e-02}$ &                    $\num{1.37e-01}\pm\scriptsize\num{2.59e-02}$ &                    $\num{1.78e-01}\pm\scriptsize\num{1.22e-02}$ & $\num{3.63e-01}\pm\scriptsize\num{1.09e-02}$ \\
                Perm5D &                    $\num{4.06e-04}\pm\scriptsize\num{1.70e-04}$ &                    $\num{2.58e-04}\pm\scriptsize\num{1.13e-04}$ & $\winc\num{7.76e-05}\pm\scriptsize\num{3.19e-05}$ &                    $\num{1.80e-03}\pm\scriptsize\num{4.44e-04}$ & $\winc\num{7.79e-05}\pm\scriptsize\num{4.19e-05}$ & $\winc\num{7.11e-05}\pm\scriptsize\num{1.45e-05}$ &                    $\num{6.96e-04}\pm\scriptsize\num{2.20e-04}$ &                    $\num{1.73e-03}\pm\scriptsize\num{4.55e-04}$ &                    $\num{2.74e-03}\pm\scriptsize\num{5.20e-04}$ &                    $\num{2.50e-03}\pm\scriptsize\num{5.58e-04}$ &                    $\num{2.06e-04}\pm\scriptsize\num{7.03e-05}$ & $\num{4.62e-04}\pm\scriptsize\num{1.20e-04}$ \\ 
                 BNN5D & $\winc\num{6.60e-02}\pm\scriptsize\num{4.03e-02}$ & $\winc\num{3.77e-02}\pm\scriptsize\num{1.89e-02}$ &   $\num{1.16e-01}\pm\scriptsize\num{8.63e-02}$ & $\winc\num{4.53e-02}\pm\scriptsize\num{3.04e-02}$ &   $\num{2.37e-01}\pm\scriptsize\num{8.04e-02}$ &   $\num{2.04e-01}\pm\scriptsize\num{9.29e-02}$ & $\winc\num{6.32e-02}\pm\scriptsize\num{5.28e-02}$ & $\winc\num{7.92e-02}\pm\scriptsize\num{5.34e-02}$ &   $\num{2.70e-01}\pm\scriptsize\num{8.78e-02}$ &   $\num{2.36e-01}\pm\scriptsize\num{8.27e-02}$ & $\winc\num{2.23e-02}\pm\scriptsize\num{6.42e-03}$ &   $\num{5.42e-01}\pm\scriptsize\num{9.21e-02}$ \\
                 \midrule
     \emph{Average Regret 5D} & $\winc\num{3.62e-02}\pm\scriptsize\num{8.99e-03}$ & $\winc\num{2.91e-02}\pm\scriptsize\num{5.46e-03}$ &   $\num{5.71e-02}\pm\scriptsize\num{1.76e-02}$ &   $\num{6.33e-02}\pm\scriptsize\num{6.99e-03}$ &   $\num{5.67e-02}\pm\scriptsize\num{1.62e-02}$ &   $\num{5.92e-02}\pm\scriptsize\num{1.87e-02}$ &   $\num{5.19e-02}\pm\scriptsize\num{1.14e-02}$ &   $\num{7.62e-02}\pm\scriptsize\num{1.17e-02}$ &   $\num{8.26e-02}\pm\scriptsize\num{1.82e-02}$ &   $\num{7.59e-02}\pm\scriptsize\num{1.73e-02}$ &   $\num{4.16e-02}\pm\scriptsize\num{2.76e-03}$ &   $\num{1.93e-01}\pm\scriptsize\num{1.86e-02}$ \\
     \midrule
     \midrule
               Levy10D & $\winc\num{6.27e-03}\pm\scriptsize\num{2.22e-03}$ & $\winc\num{6.27e-03}\pm\scriptsize\num{2.22e-03}$ & $\num{1.04e-02}\pm\scriptsize\num{2.10e-03}$ & $\num{1.04e-02}\pm\scriptsize\num{2.10e-03}$ &                    $\num{2.16e-02}\pm\scriptsize\num{3.71e-03}$ &                    $\num{2.17e-02}\pm\scriptsize\num{5.30e-03}$ &                    $\num{8.65e-02}\pm\scriptsize\num{2.01e-02}$ &                    $\num{1.46e-01}\pm\scriptsize\num{1.41e-02}$ & $\winc\num{6.21e-03}\pm\scriptsize\num{2.48e-03}$ & $\winc\num{5.81e-03}\pm\scriptsize\num{1.99e-03}$ & $\winc\num{6.16e-03}\pm\scriptsize\num{8.94e-04}$ & $\num{1.06e-01}\pm\scriptsize\num{7.64e-03}$ \\
         Rosenbrock10D & $\winc\num{2.34e-03}\pm\scriptsize\num{1.43e-03}$ &                    $\num{2.01e-03}\pm\scriptsize\num{6.91e-04}$ & $\winc\num{9.14e-04}\pm\scriptsize\num{1.25e-04}$ &                    $\num{5.67e-03}\pm\scriptsize\num{1.60e-03}$ &                    $\num{2.25e-03}\pm\scriptsize\num{2.58e-04}$ &                    $\num{4.96e-03}\pm\scriptsize\num{4.40e-04}$ &                    $\num{1.42e-02}\pm\scriptsize\num{4.43e-03}$ &                    $\num{7.65e-02}\pm\scriptsize\num{1.03e-02}$ &                    $\num{5.10e-03}\pm\scriptsize\num{1.44e-03}$ &                    $\num{5.00e-03}\pm\scriptsize\num{1.70e-03}$ &                    $\num{3.09e-03}\pm\scriptsize\num{5.77e-04}$ & $\num{2.82e-02}\pm\scriptsize\num{3.92e-03}$ \\
         G-Function10D &                    $\num{2.92e-01}\pm\scriptsize\num{3.85e-02}$ &                    $\num{3.53e-01}\pm\scriptsize\num{2.74e-02}$ &                    $\num{3.79e-01}\pm\scriptsize\num{2.24e-02}$ &                    $\num{4.21e-01}\pm\scriptsize\num{2.35e-02}$ & $\winc\num{1.79e-01}\pm\scriptsize\num{2.54e-02}$ &                    $\num{4.15e-01}\pm\scriptsize\num{1.12e-02}$ &                    $\num{3.24e-01}\pm\scriptsize\num{2.28e-02}$ &                    $\num{3.33e-01}\pm\scriptsize\num{2.06e-02}$ &                    $\num{2.53e-01}\pm\scriptsize\num{3.76e-02}$ &                    $\num{2.55e-01}\pm\scriptsize\num{3.72e-02}$ &                    $\num{3.80e-01}\pm\scriptsize\num{1.34e-02}$ & $\num{4.50e-01}\pm\scriptsize\num{6.48e-03}$ \\
               Perm10D & $\num{3.74e-04}\pm\scriptsize\num{1.26e-04}$ & $\num{4.27e-04}\pm\scriptsize\num{1.34e-04}$ & $\winc\num{3.59e-04}\pm\scriptsize\num{2.13e-04}$ & $\num{6.52e-04}\pm\scriptsize\num{2.04e-04}$ & $\num{3.37e-04}\pm\scriptsize\num{8.49e-05}$ & $\num{5.53e-04}\pm\scriptsize\num{1.33e-04}$ &                    $\num{1.01e-03}\pm\scriptsize\num{3.10e-04}$ &                    $\num{1.48e-03}\pm\scriptsize\num{3.92e-04}$ & $\num{4.07e-04}\pm\scriptsize\num{1.21e-04}$ & $\num{4.08e-04}\pm\scriptsize\num{1.48e-04}$ & $\num{5.57e-04}\pm\scriptsize\num{1.43e-04}$ & $\winc\num{1.81e-04}\pm\scriptsize\num{5.44e-05}$ \\
                BNN10D & $\winc\num{1.23e-01}\pm\scriptsize\num{3.76e-02}$ & $\winc\num{1.00e-01}\pm\scriptsize\num{3.43e-02}$ &   $\num{1.96e-01}\pm\scriptsize\num{5.16e-02}$ &   $\num{1.68e-01}\pm\scriptsize\num{4.09e-02}$ & $\winc\num{1.45e-01}\pm\scriptsize\num{3.60e-02}$ &   $\num{1.61e-01}\pm\scriptsize\num{2.86e-02}$ & $\winc\num{1.51e-01}\pm\scriptsize\num{4.27e-02}$ & $\winc\num{1.13e-01}\pm\scriptsize\num{4.00e-02}$ &   $\num{2.58e-01}\pm\scriptsize\num{4.96e-02}$ &   $\num{2.02e-01}\pm\scriptsize\num{3.79e-02}$ & $\winc\num{8.65e-02}\pm\scriptsize\num{2.29e-02}$ &   $\num{5.92e-01}\pm\scriptsize\num{5.34e-02}$ \\
                \midrule
    \emph{Average Regret 10D} & $\winc\num{8.48e-02}\pm\scriptsize\num{1.08e-02}$ &   $\num{9.24e-02}\pm\scriptsize\num{8.79e-03}$ &   $\num{1.17e-01}\pm\scriptsize\num{1.13e-02}$ &   $\num{1.21e-01}\pm\scriptsize\num{9.45e-03}$ & $\winc\num{6.97e-02}\pm\scriptsize\num{8.84e-03}$ &   $\num{1.21e-01}\pm\scriptsize\num{6.24e-03}$ &   $\num{1.15e-01}\pm\scriptsize\num{1.05e-02}$ &   $\num{1.34e-01}\pm\scriptsize\num{9.65e-03}$ &   $\num{1.05e-01}\pm\scriptsize\num{1.25e-02}$ &   $\num{9.36e-02}\pm\scriptsize\num{1.06e-02}$ &   $\num{9.52e-02}\pm\scriptsize\num{5.30e-03}$ &   $\num{2.35e-01}\pm\scriptsize\num{1.09e-02}$ \\
    \midrule
    \midrule
               Levy20D & $\winc\num{1.51e-02}\pm\scriptsize\num{1.69e-03}$ & $\winc\num{1.40e-02}\pm\scriptsize\num{1.63e-03}$ & $\winc\num{1.98e-02}\pm\scriptsize\num{8.61e-03}$ & $\winc\num{2.64e-02}\pm\scriptsize\num{1.12e-02}$ &                    $\num{4.27e-02}\pm\scriptsize\num{4.16e-03}$ &                    $\num{6.91e-02}\pm\scriptsize\num{9.00e-03}$ &                    $\num{1.88e-01}\pm\scriptsize\num{1.15e-02}$ &                    $\num{2.01e-01}\pm\scriptsize\num{1.07e-02}$ & $\winc\num{1.13e-02}\pm\scriptsize\num{4.60e-03}$ & $\winc\num{1.61e-02}\pm\scriptsize\num{5.47e-03}$ & $\winc\num{1.98e-02}\pm\scriptsize\num{7.88e-03}$ & $\num{1.48e-01}\pm\scriptsize\num{6.58e-03}$ \\
         Rosenbrock20D &                    $\num{3.47e-02}\pm\scriptsize\num{7.08e-03}$ &                    $\num{6.03e-03}\pm\scriptsize\num{9.93e-04}$ &                    $\num{8.94e-03}\pm\scriptsize\num{4.00e-03}$ &                    $\num{1.91e-02}\pm\scriptsize\num{4.04e-03}$ &                    $\num{7.41e-03}\pm\scriptsize\num{1.14e-03}$ &                    $\num{7.61e-03}\pm\scriptsize\num{2.15e-03}$ &                    $\num{6.46e-02}\pm\scriptsize\num{1.22e-02}$ &                    $\num{1.41e-01}\pm\scriptsize\num{1.29e-02}$ & $\winc\num{2.96e-03}\pm\scriptsize\num{1.36e-04}$ & $\winc\num{4.27e-03}\pm\scriptsize\num{1.33e-03}$ &                    $\num{1.09e-02}\pm\scriptsize\num{1.52e-03}$ & $\num{7.80e-02}\pm\scriptsize\num{8.38e-03}$ \\
         G-Function20D &                    $\num{4.16e-01}\pm\scriptsize\num{8.99e-03}$ &                    $\num{4.18e-01}\pm\scriptsize\num{1.70e-02}$ &                    $\num{4.59e-01}\pm\scriptsize\num{6.77e-03}$ &                    $\num{4.86e-01}\pm\scriptsize\num{3.95e-03}$ &                    $\num{4.70e-01}\pm\scriptsize\num{4.43e-03}$ &                    $\num{4.92e-01}\pm\scriptsize\num{1.58e-03}$ &                    $\num{4.18e-01}\pm\scriptsize\num{1.33e-02}$ & $\winc\num{4.02e-01}\pm\scriptsize\num{1.61e-02}$ & $\winc\num{3.79e-01}\pm\scriptsize\num{2.97e-02}$ & $\winc\num{3.73e-01}\pm\scriptsize\num{2.56e-02}$ &                    $\num{4.47e-01}\pm\scriptsize\num{9.37e-03}$ & $\num{4.86e-01}\pm\scriptsize\num{2.44e-03}$ \\
               Perm20D &                    $\num{7.45e-05}\pm\scriptsize\num{2.09e-05}$ &                    $\num{7.46e-05}\pm\scriptsize\num{2.50e-05}$ &                    $\num{2.20e-04}\pm\scriptsize\num{8.98e-05}$ &                    $\num{1.57e-04}\pm\scriptsize\num{7.50e-05}$ &                    $\num{9.98e-05}\pm\scriptsize\num{3.19e-05}$ &                    $\num{2.03e-04}\pm\scriptsize\num{8.86e-05}$ & $\num{3.54e-05}\pm\scriptsize\num{6.52e-06}$ &                    $\num{1.85e-04}\pm\scriptsize\num{6.90e-05}$ &                    $\num{7.98e-05}\pm\scriptsize\num{2.19e-05}$ &                    $\num{9.28e-05}\pm\scriptsize\num{3.89e-05}$ &                    $\num{9.44e-05}\pm\scriptsize\num{3.25e-05}$ & $\winc\num{1.90e-05}\pm\scriptsize\num{4.67e-06}$ \\
                Bnn20D & $\winc\num{1.58e-01}\pm\scriptsize\num{4.12e-02}$ & $\winc\num{1.23e-01}\pm\scriptsize\num{3.21e-02}$ &   $\num{1.84e-01}\pm\scriptsize\num{3.46e-02}$ & $\winc\num{1.42e-01}\pm\scriptsize\num{2.70e-02}$ &   $\num{1.77e-01}\pm\scriptsize\num{3.46e-02}$ &   $\num{2.45e-01}\pm\scriptsize\num{4.41e-02}$ &   $\num{1.89e-01}\pm\scriptsize\num{3.98e-02}$ &   $\num{3.05e-01}\pm\scriptsize\num{7.02e-02}$ &   $\num{2.93e-01}\pm\scriptsize\num{5.72e-02}$ &   $\num{3.05e-01}\pm\scriptsize\num{5.01e-02}$ & $\winc\num{1.11e-01}\pm\scriptsize\num{2.06e-02}$ &   $\num{6.85e-01}\pm\scriptsize\num{3.29e-02}$ \\
                \midrule
    \emph{Average Regret 20D} & $\winc\num{1.25e-01}\pm\scriptsize\num{8.57e-03}$ & $\winc\num{1.12e-01}\pm\scriptsize\num{7.27e-03}$ &   $\num{1.34e-01}\pm\scriptsize\num{7.31e-03}$ &   $\num{1.35e-01}\pm\scriptsize\num{5.95e-03}$ &   $\num{1.39e-01}\pm\scriptsize\num{7.03e-03}$ &   $\num{1.63e-01}\pm\scriptsize\num{9.02e-03}$ &   $\num{1.72e-01}\pm\scriptsize\num{9.03e-03}$ &   $\num{2.10e-01}\pm\scriptsize\num{1.48e-02}$ &   $\num{1.37e-01}\pm\scriptsize\num{1.29e-02}$ &   $\num{1.40e-01}\pm\scriptsize\num{1.13e-02}$ & $\winc\num{1.18e-01}\pm\scriptsize\num{4.81e-03}$ &   $\num{2.80e-01}\pm\scriptsize\num{6.94e-03}$ \\
    \midrule
    \bottomrule
    \end{tabular}
